Understanding Reduced-Voltage Operation in Modern DRAM Chips: Characterization, Analysis, and Mechanisms

The energy consumption of DRAM is a critical concern in modern computing systems. Improvements in manufacturing process technology have allowed DRAM vendors to lower the DRAM supply voltage conservatively, which reduces some of the DRAM energy consumption. We would like to reduce the DRAM supply voltage more aggressively, to further reduce energy. Aggressive supply voltage reduction requires a thorough understanding of the effect voltage scaling has on DRAM access latency and DRAM reliability. In this paper, we take a comprehensive approach to understanding and exploiting the latency and reliability characteristics of modern DRAM when the supply voltage is lowered below the nominal voltage level specified by DRAM standards. Using an FPGA-based testing platform, we perform an experimental study of 124 real DDR3L (low-voltage) DRAM chips manufactured recently by three major DRAM vendors. We find that reducing the supply voltage below a certain point introduces bit errors in the data, and we comprehensively characterize the behavior of these errors. We discover that these errors can be avoided by increasing the latency of three major DRAM operations (activation, restoration, and precharge). We perform detailed DRAM circuit simulations to validate and explain our experimental findings. We also characterize the various relationships between reduced supply voltage and error locations, stored data patterns, DRAM temperature, and data retention. Based on our observations, we propose a new DRAM energy reduction mechanism, called Voltron. The key idea of Voltron is to use a performance model to determine by how much we can reduce the supply voltage without introducing errors and without exceeding a user-specified threshold for performance loss. Voltron reduces the average system energy by 7.3% while limiting the average system performance loss to only 1.8%, for a variety of workloads.

==> sections/a.tex <==
% !TEX root=../paper.tex

\appendix
\label{sec:appendix}

\section*{Appendix}


\section{FPGA Schematic of DRAM Power Pins}
\label{sec:pin_layout}

\fix{\figref{pin_layout} shows a schematic of the DRAM pins that our FPGA
board~\cite{ml605_schematic} connects to (see \secref{fpga} for our experimental
methodology). Since there are a large number of pins that are used for different
purposes (e.g., data address), we zoom in on the right side of the figure to
focus on the power pins that we adjust for our experiments in this paper.}
\fixIII{Power pin numbering information can be found on the datasheets provided
  by all major vendors (e.g., \cite{micronDDR3L_2Gb, hynix-ddr3l,
    samsungddr3l_2Gb}).} In particular, we tune the VCC1V5 pin \fix{on the
  FPGA}, which is directly connected to all of the $V_{DD}$ and $V_{DDQ}$ pins
on the DIMM. The reference voltage VTTVREF is automatically adjusted by the DRAM
to half of VCC1V5.

\figputHS{pin_layout}{0.7}{DRAM power pins \fix{controlled by the ML605 FPGA board}.}


\section{Effect of Data Pattern on Error Rate}
\label{sec:datapatt}

\fix{As
discussed in \ssecref{volt_sensitivity}, we do \emph{not} observe a significant
effect \fix{of} different stored data patterns \fix{on the DRAM error rate when we
  reduce the supply voltage.} \figref{datapatt} shows the average bit error rate
(BER) of three different data patterns (\patt{aa}, \patt{cc}, and \patt{ff})
across different supply voltage levels for each vendor. Each data pattern
represents the byte value (shown in hex) that we fill into the DRAM. The error
bars indicate the 95\% confidence interval.  We make two observations from the
figure.

%For each shown data pattern, we also test its bit inversion in the same experiment,
%as discussed in \ssecref{dramtest}.

%\figputWL{datapatt/alt_patt_temp20_trcd4_trp4}{Effect of data patterns on BERs
%  across different supply voltage levels.}{datapatt}

\figputHSL{datapatt/alt_patt_temp20_trcd4_trp4}{0.72}{datapatt}{Effect of
  \fixIII{stored
    data pattern} on \fix{bit error rate (BER)} across different supply voltage levels.}

First, the BER increases as we reduce the supply
voltage for all three data patterns. We made a similar observation in
\ssecref{volt_sensitivity}, which shows that the fraction of errors increases as the
supply voltage drops. We explained our hypothesis on the cause of the errors, and
used both experiments and simulations to test the
hypothesis, in \ssecref{low_volt_latency}.

Second, we do \emph{not} observe a significant difference across the BER values from
the three different data patterns. We attempt to answer the following question:
\fix{Do} different data patterns induce BER values that are statistically different
from each other at each voltage level? To answer this, we conduct a one-way
ANOVA (analysis of variance) test across the measured BERs from all three data patterns at each supply
voltage level to calculate a \emph{p-value}. If the p-value is below 0.05, we
can claim that these three data patterns induce a statistically-significant
difference on the error rate. \tabref{pval} shows the calculated p-value at each
supply voltage level. At certain supply voltage levels, we do not have a p-value
listed (shown as --- or $\triangle$ in the table), \fixIII{either} because there
are no errors \fixIV{(indicated as ---)} or we cannot
reliably access data \fixIV{from the DIMMs} even if the access latency is
higher than the standard value \fixIV{(indicated as $\triangle$)}.

%The test reports a
%\emph{p-value}, which is probability vaindicates the probability of

\input{sections/tables/data_patt_pvalue}

Using the one-way ANOVA test, we find that using different data patterns does
\emph{not} have a statistically significant (i.e., p-value $\geq$ 0.05) effect
on the error rate at \emph{all} supply voltage levels. Significant effects
(i.e., p-value < 0.05) occur at 1.100V for Vendor~A, at 1.025V for Vendor~B, and
at both 1.250V and 1.100V for Vendor~C. As a result, our study does \emph{not}
\fixIV{provide} enough evidence to conclude that using any of the three data
patterns (\patt{aa}, \patt{cc}, and \patt{ff}) induces higher or lower error
rates than the other two patterns at reduced voltage levels. }

%The one-way ANOVA tests the null hypothesis that two or more groups have the
%same population mean
%
%P-values for the Shapiro-Wilk test of normality and the BrownForsythe test for
%homogeneity of variance. A p-value less that α = 0.05 is sufficient to reject
%the null hypothesis (indicated in bold). Shapiro-Wilk tests the null hypothesis
%that the data are drawn from a normal distribution. BrownForsythe tests whether
%the one-time randomization and re-randomization samples are drawn from
%distributions with the same variance. Boldface indicates statistically
%significant non-normal execution times and unequal variances, respectively.
%Section 5.1 explores these results further.
%
%They start with the null hypothesis that the 2 populations are identical, then
%try to reject that hypothesis. We can never prove the null to be true, just
%reject it,
%
%but we cannot prove that they are the same
%
%conclusion: we cannot conclude that using different stored data patterns lead
%to different error rates under reduced voltage.

\fix{
\section{SPICE Simulation Model}
\label{spice_model}

We perform circuit-level SPICE simulations to understand in detail how the DRAM cell
arrays operate at low supply voltage. We model a DRAM cell array in SPICE,
and simulate its behavior for different supply voltages. We have released our
SPICE model online~\cite{volt-github}.

\paratitle{DRAM Cell Array Model} We build a detailed cell array model, as shown
in \figref{spice_model}. In the cell array, the DRAM cells are organized as $512
x 512$ array, which is a common organization in modern DRAM
chips~\cite{vogelsang-micro2010}. Each column is vertical, and corresponds to
512~cells sharing a bitline that connects to a sense amplifier. Due to the
bitline wire and the cells that are connected to the bitline, there is parasitic
resistance and capacitance on each bitline. Each row consists of 512~cells
sharing the same wordline, which also has parasitic resistance and capacitance.
The amount of parasitic resistance and capacitance on the bitlines and wordlines
is a major factor that affects the latency of DRAM operations accessing a cell
array~\cite{lee-hpca2013,lee-sigmetrics2017}.

%Horizontally located 512 cells share the same wordline that
%is connected to a wordline driver.
%Similar to the bitlines, each wordline
%also has parasitic resistance and capacitance. The parasitic resistance and
%capacitance affects the operation of the DRAM cell array.

\figputHS{spice_model}{1.0}{Our SPICE model \fixIV{schematic} of a DRAM cell array.}

\paratitle{Simulation Methodology} We use the LTspice~\cite{ltspice} SPICE simulator
to perform our simulations.
To find the access latency of the DRAM
operations under different supply voltages, we build a DRAM cell array using
technology parameters that we derive from a \SI{55}{\nano\meter} DRAM
model~\cite{vogelsang-micro2010} and from a \SI{45}{\nano\meter} process technology model~\cite{ptm,
  zhao-isqed2006}. By default, we assume that the cell capacitance is \SI{24}{\femto\farad} and
the bitline capacitance is \SI{144}{\femto\farad}~\cite{vogelsang-micro2010}. The nominal
\varr is 1.35V, and we perform simulations to obtain the latency of DRAM operations
at every 25mV step from 1.35V down to 0.9V.  The results of our SPICE simulations
are discussed in Section~\ref{ssec:volt_sensitivity} and \ref{ssec:low_volt_latency}.
}

%The
%nominal sense amplifier operating voltage is 1.35V, and the wordlines drive
%3.0V when asserted.
%%In our simulations, we issue an \act command at $0 ns$ and \pre command at
%%$25 ns$, unless stated otherwise.
%We simulate the access latency of the model under different sense amplifier
%operating voltages ranging from 0.9V to 1.35V.

\newpage

\section{Spatial Distribution of Errors}
\label{spatial}

In this section, we expand upon the spatial locality data presented in
\ssecref{spatial}. \fix{Figures~\ref{fig:full_loc_A}, \ref{fig:full_loc_B}, and
\ref{fig:full_loc_C} show the physical locations of errors that occur when the
supply voltage is reduced for a representative DIMM from Vendors~A, B, and C,
respectively.} At higher voltage levels, even if errors occur, they
tend to cluster in certain regions of a DIMM. However, as we reduce the supply
voltage further, the number of errors increases, and the errors start to spread
across the \fix{entire} DIMM.

\begin{figure}[!h]
    \centering
    \subcaptionbox{Supply voltage=1.075V.}[0.49\linewidth][l]
    {
        %\includegraphics[width=0.8\linewidth]{plots/figs/{crucialb41_rcd4_rp4_ret0_temp20_volt1.075000_fix_row}.pdf}
        %\includegraphics[width=0.49\linewidth]{plots/figs/add_eq/{crucialb41_rcd4_rp4_ret0_temp20_volt1.075000_fix_row_addeq}.pdf}
        \includegraphics[width=0.49\linewidth]{plots/figs/add_eq/crucial_1075.pdf}
    }
    \subcaptionbox{Supply voltage=1.1V.}[0.49\linewidth][r]
    {
        %\includegraphics[width=0.8\linewidth]{plots/figs/{crucialb41_rcd4_rp4_ret0_temp20_volt1.100000_fix_row}.pdf}
        %\includegraphics[width=0.49\linewidth]{plots/figs/add_eq/{crucialb41_rcd4_rp4_ret0_temp20_volt1.100000_fix_row_addeq}.pdf}
        \includegraphics[width=0.49\linewidth]{plots/figs/add_eq/crucial_110.pdf}
    }

    %\subcaptionbox{1.15V.}[0.8\linewidth][l]
    %{
    %    %\includegraphics[width=0.8\linewidth]{plots/figs/add_eq/{crucialb41_rcd4_rp4_ret0_temp20_volt1.150000_fix_row_addeq}.pdf}
    %    \includegraphics[scale=0.5]{plots/figs/{crucialb41_rcd4_rp4_ret0_temp20_volt1.150000_fix_row}.pdf}
    %}
    \caption{Probability of error occurrence due to \fixIV{reduced-voltage operation} in a DIMM from \fix{Vendor~A}.}
    \label{fig:full_loc_A}
\end{figure}

\begin{figure}[!h]
    \centering
    \subcaptionbox{Supply voltage=1.025V.}[0.49\linewidth][l]
    {
        %\includegraphics[width=0.47\linewidth]{plots/figs/add_eq/{samsungo13_rcd4_rp4_ret0_temp20_volt1.025000_fix_row_addeq}.pdf}
        \includegraphics[width=0.47\linewidth]{plots/figs/add_eq/samsung_1025}
    }
    \subcaptionbox{Supply voltage=1.05V.}[0.49\linewidth][r]
    {
        %\includegraphics[width=0.47\linewidth]{plots/figs/add_eq/{samsungo13_rcd4_rp4_ret0_temp20_volt1.050000_fix_row_addeq}.pdf}
        \includegraphics[width=0.47\linewidth]{plots/figs/add_eq/samsung_105}
    }

    \subcaptionbox{Supply voltage=1.1V.}[0.8\linewidth][c]
    {
        %\includegraphics[width=0.49\linewidth]{plots/figs/add_eq/{samsungo13_rcd4_rp4_ret0_temp20_volt1.100000_fix_row_addeq}.pdf}
        \includegraphics[width=0.47\linewidth]{plots/figs/add_eq/samsung_110}
    }
    \caption{Probability of error occurrence due to \fixIV{reduced-voltage operation} in a DIMM from \fix{Vendor~B}.}
    \label{fig:full_loc_B}
\end{figure}

\begin{figure}[!h]
    \centering
    \subcaptionbox{Supply voltage=1.1V.}[0.49\linewidth][l]
    {
        %\includegraphics[width=0.47\linewidth]{plots/figs/add_eq/{hynixp65_rcd4_rp4_ret0_temp20_volt1.100000_fix_row_addeq}.pdf}
        \includegraphics[width=0.47\linewidth]{plots/figs/add_eq/hynix_110}
    }
    %\subcaptionbox{1.125V.}[0.49\linewidth][l]
    %{
    %    \includegraphics[width=0.49\linewidth]{plots/figs/add_eq/{hynixp65_rcd4_rp4_ret0_temp20_volt1.125000_fix_row_addeq}.pdf}
    %}
    \subcaptionbox{Supply voltage=1.15V.}[0.49\linewidth][l]
    {
        %\includegraphics[width=0.47\linewidth]{plots/figs/add_eq/{hynixp65_rcd4_rp4_ret0_temp20_volt1.150000_fix_row_addeq}.pdf}
        \includegraphics[width=0.47\linewidth]{plots/figs/add_eq/hynix_115}
    }
    %
    %\subcaptionbox{1.175V.}[0.49\linewidth][l]
    %{
    %    \includegraphics[width=0.49\linewidth]{plots/figs/add_eq/{hynixp65_rcd4_rp4_ret0_temp20_volt1.175000_fix_row_addeq}.pdf}
    %}
    \subcaptionbox{Supply voltage=1.2V.}[0.49\linewidth][l]
    {
        %\includegraphics[width=0.49\linewidth]{plots/figs/add_eq/{hynixp65_rcd4_rp4_ret0_temp20_volt1.200000_fix_row_addeq}.pdf}
        \includegraphics[width=0.47\linewidth]{plots/figs/add_eq/hynix_120}
    }
    \caption{Probability of error occurrence due to \fixIV{reduced-voltage operation} in a DIMM from \fix{Vendor~C}.}
    \label{fig:full_loc_C}
\end{figure}

\ignore{
\begin{figure*}[!h]
    \centering
    \subcaptionbox{1.075V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{crucialb41_rcd4_rp4_ret0_temp20_volt1.075000_fix_row}.pdf}
    }
    %
    \subcaptionbox{1.1V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{crucialb41_rcd4_rp4_ret0_temp20_volt1.100000_fix_row}.pdf}
    }
    %
    \subcaptionbox{1.15V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{crucialb41_rcd4_rp4_ret0_temp20_volt1.150000_fix_row}.pdf}
    }
    \caption{Probability of error occurrence due to low voltage in a DIMM from vendor A.}
    \label{fig:full_loc_A}
\end{figure*}

\begin{figure*}[!h]
    \centering
    \subcaptionbox{1.025V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{samsungo13_rcd4_rp4_ret0_temp20_volt1.025000_fix_row}.pdf}
    }
    \subcaptionbox{1.05V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{samsungo13_rcd4_rp4_ret0_temp20_volt1.050000_fix_row}.pdf}
    }
    \subcaptionbox{1.1V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{samsungo13_rcd4_rp4_ret0_temp20_volt1.100000_fix_row}.pdf}
    }
    \caption{Probability of error occurrence due to low voltage in a DIMM from vendor B.}
    \label{fig:full_loc_B}
\end{figure*}

\begin{figure*}[!h]
    \centering
    \subcaptionbox{1.1V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{hynixp65_rcd4_rp4_ret0_temp20_volt1.100000_fix_row}.pdf}
    }
    \subcaptionbox{1.125V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{hynixp65_rcd4_rp4_ret0_temp20_volt1.125000_fix_row}.pdf}
    }
    \subcaptionbox{1.15V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{hynixp65_rcd4_rp4_ret0_temp20_volt1.150000_fix_row}.pdf}
    }
    %
    \subcaptionbox{1.175V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{hynixp65_rcd4_rp4_ret0_temp20_volt1.175000_fix_row}.pdf}
    }
    \subcaptionbox{1.2V.}[0.31\linewidth][l]
    {
        \includegraphics[width=0.31\linewidth]{plots/figs/{hynixp65_rcd4_rp4_ret0_temp20_volt1.200000_fix_row}.pdf}
    }
    \caption{Probability of error occurrence due to low voltage in a DIMM from vendor C.}
    \label{fig:full_loc_C}
\end{figure*}
}

\newpage
\
\newpage

\section{Full Information of Every Tested DIMM}
\label{sec:dimm_info}

\tabref{modules} lists the parameters of every DRAM module that we evaluate,
\fixIII{along with the \vmin we discovered for each module based on our
  experimental characterization (\ssecref{volt_sensitivity}).} \fix{We provide
  all results for all DIMMs in our GitHub repository~\cite{volt-github}.}
\input{sections/tables/modules}
\vspace{0.1in}


==> sections/cell_ops <==
\section{DRAM Cell Operation}
\label{dram_cell_op}

In this section, we explain the how the DRAM cell and its state change during
the three fundamental operations: activation, restoration, and precharge
(see \ssecref{access_data}).
\figref{dram_curve} shows the bitline voltage level during these operations with
\vdd set to 1.35V. An \act command and a \pre command are issued at 0ns and 50ns,
respectively. To further help understand the operations, we use
\figref{dram_state} to describe the state of the cell, bitline, and sense
amplifier during the same time frame as \figref{dram_curve}. A bitline is used
to connect a cell with its sense amplifier (in the row buffer) for data
accesses. Accessing data in a DRAM cell consists of four major steps:

\begin{figure}[!h]
    \centering
   \subcaptionbox{DRAM bitline voltage.\label{fig:dram_curve}}
    {
        \includegraphics[scale=0.8]{plots/dram_curve}
    }
    %
    \subcaptionbox{DRAM state.\label{fig:dram_state}}
    {
        \includegraphics[scale=0.8]{plots/dram_state}
    }
    \caption{DRAM phases during a DRAM access.}
\end{figure}

\paratitle{Precharge} Initially, each cell in the DRAM is in a charged
state (for data value 1) or a discharged state (for data value 0) at 0ns ($T0$). The
amount of filled gray color represents the amount of charge in the cell. In our
shown example, we assume the cell is fully charged, storing a data value of 1.
The bitline voltage is maintained at a voltage of $\frac{1}{2}$\vdd.

\paratitle{Charge Sharing} An \act command connects a row of cells to their
bitlines. This triggers the charge stored in the cells to start flowing to the
bitlines (or the other way around, depending on the initial charge level in the
cell) via a process called \emph{charge sharing} (at time $T1$). In our example,
the cell is initially charged. Hence, it perturbs the bitline's voltage from
$\frac{1}{2}$\vdd to $\frac{1}{2}$\vdd$+\delta$ by a small amount of charge
($\delta$).

\paratitle{Sensing and Amplification} After the charge sharing phase, the
sense amplifier senses the voltage perturbation on the bitline towards either
\vdd or 0. Following the same direction, it starts to amplify the bitline
voltage by injecting more charge into the bitline and the cell. When
the bitline voltage surpasses 75\% of \vdd (at time $T2$), the binary data becomes latched in
the sense amplifier, thus ensuring that the correct data can be read by a \crd
command. These two phases are also known as the activation phase. The activation
latency is the time elapsed from $T0$ to $T2$, which is defined as \trcd.

\paratitle{Restoration} After the row is activated and each sense
amplifier latches in the binary data of its cell, the DRAM starts to restore the
connected cell's charge back to its original fully-charged state (at time $T3$).
This phase is known as restoration, and its latency (from $T0$ to $T3$) is
defined as \tras.

To activate a different row of cells within the same array of the activated row,
the memory controller sends a \pre command to disconnect the cells from the
bitline. Then, the sense amplifier brings the bitline back to $\frac{1}{2}$\vdd
(at time $T4$). The precharge latency is defined at \trp, from the issue time of
\pre (50ns) to $T4$.




==> sections/spice_exp.tex <==
To further understand the relationship between access latency and voltage,
we express the access latency as a mathematical function. Since the SPICE
simulation employs a series of circuit
models~\cite{nagel-spice,massobrio1993semiconductor}, we can simplify the
latency growth function with only the \vdd parameter given \emph{our}
specific transistor, resistance, and capacitance parameters. \sg{this is
unclear still - what is the latency growth function?}

We represent the latency as an exponential function of \varr
%(abbreviated as $V$)
in Equation~\ref{exp_decay}. $\lambda$ is the decay rate of the latency,  and
$y_{0}$ represents the initial latency value when \varr is 0, with an offset of
$\epsilon$. In this work, we bound the value of \varr from 0.9V to 1.35V for our
SPICE simulations.

\vspace{-0.15in}
\begin{align}
    y(V_{array})=y_{0} \cdot e^{-\lambda V_{array}} + \epsilon
    \label{exp_decay}
\end{align}
\vspace{-0.15in}

\tabref{exp_func_params} shows the coefficients of the exponential function
after fitting the function to our SPICE simulation results. We calculate the
coefficients using the SciPy~\cite{scipy} non-linear regression, which minimizes
least squares. To measure how well the regression function fits to the SPICE
results, we report $R^2$, which ranges from 0\% (i.e., does not fit at all) to
100\% (i.e., a perfect fit). Our exponential function matches very closely with
our SPICE simulation results, with a 99.91\% and 99.85\% $R^2$ for the activation
and precharge latencies, respectively.

\begin{table}[h]
    \renewcommand{\arraystretch}{0.9}
    \small
    \centering
    \setlength{\tabcolsep}{.7em}
    \begin{tabular}{crrrc}
        \toprule
        \textbf{Latency} & \multicolumn{1}{c}{$y_{0}$} & \multicolumn{1}{c}{$\lambda$} & \multicolumn{1}{c}{$\epsilon$} & \multicolumn{1}{c}{$R^{2}$ (\%)}\\
        \midrule
        Activation & 9471.58 & 7.15 & 6.72 & \textbf{99.91} \\
        Precharge & 26299.34 & 8.33 & 7.71 & \textbf{99.85} \\
        \bottomrule
    \end{tabular}
    \caption{Coefficients and goodness of fit of Equation~\ref{exp_decay}.}
    \label{tab:exp_func_params}
\end{table}

Our SPICE simulations not only
validate that a lower supply voltage requires longer access latency, but also provide
us with a model that generates much more precise latency values given a certain
supply voltage.

%%%%% END SPICE MODEL %%%%%


==> sections/subplots/loc_samsung.tex <==
\begin{figure}[!h]
    \centering
    \subcaptionbox{1.05V}[\linewidth]
    {
        \includegraphics{plots/figs/{samsungo13_rcd4_rp4_ret0_temp20_volt1.050000_fix_row}.pdf}
    }

    \subcaptionbox{1.025V}[\linewidth]
    {
        \includegraphics{plots/figs/{samsungo13_rcd4_rp4_ret0_temp20_volt1.025000_fix_row}.pdf}
    }
    \caption{Spatial distribution of errors in a Vendor B's DIMM.}
    \label{fig:locality_B}
\end{figure}


==> sections/subplots/motivation.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    {
        \includegraphics[width=\linewidth]{plots/powerbreakdown/power_breakdown_Freq_power_isca}
        \vspace{-0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/powerbreakdown/power_breakdown_Freq_energy_isca}
        \vspace{-0.1in}
    }

    \caption{Power and energy consumption due to different DRAM frequency.}
    \label{fig:voltron}
\end{figure}


==> sections/subplots/voltron.tex <==
\begin{figure}[!h]
    \centering
    \captionsetup[subfigure]{justification=centering}
    %\subcaptionbox{1}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/voltron_perfloss}
        %\includegraphics[scale=1.0]{plots/voltron_perfloss}
        \vspace{-0.1in}
    }

    %\subcaptionbox{2}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/voltron_dramenergysavings}
        %\includegraphics[scale=1.0]{plots/voltron_dramenergysavings}
        \vspace{-0.1in}
    }

    %\subcaptionbox{3}[\linewidth]
    {
        \includegraphics[width=\linewidth]{plots/voltron_sysenergysavings}
        %\includegraphics[scale=1.0]{plots/voltron_sysenergysavings}
        %\vspace{-0.1in}
    }
    \vspace{-0.1in}
    \caption{Comparison between \voltron and an oracle with a system performance
      loss bound of 5\%.}
    \label{fig:voltron}
\end{figure}


==> sections/subplots/voltron_interval.tex <==
\begin{figure}[!h]
    \centering
    %\captionsetup[subfigure]{justification=left}
    %\subcaptionbox{1}[\linewidth]

    \subcaptionbox*{}[0.49\linewidth][l]
    {
      \includegraphics[scale=1]{sim_results/paper_plots/voltron_homo_intervals/voltron_intervals_drampowersavings}
    }
    \subcaptionbox*{}[0.49\linewidth][r]
    {
      \includegraphics[scale=1]{sim_results/paper_plots/voltron_homo_intervals/voltron_intervals_perfwattgains}
    }
    \vspace{-0.25in}

    \caption{\response{Performance sensitivity of \voltron to profile intervals.}}}
    \label{fig:interval}
\end{figure}


==> sections/subplots/vsweep.tex <==
% plots/vsweep_norm_dram_energy.pdf  plots/vsweep_norm_ipc.pdf
% plots/vsweep_norm_system_energy.pdf  plots/vsweep_norm_ws.pdf
\begin{figure*}[t]
    \centering
    \captionsetup[subfigure]{justification=centering}
    {
        \includegraphics[width=\linewidth]{plots/vsweep_norm_ipc}
        \vspace{-0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/vsweep_norm_dram_energy}
        \vspace{-0.1in}
    }

    {
        \includegraphics[width=\linewidth]{plots/vsweep_norm_system_energy}
        \vspace{-0.1in}
    }
    \caption{Impact of adjusting DRAM array voltage on system performance and energy
    savings.}
    \label{fig:vsweep}
\end{figure*}


==> sections/tables/ecc.tex <==
\begin{table}[h]
%\reftiny
  \centering
    \setlength{\tabcolsep}{.65em}
    \begin{tabular}{ccrrrrr}
        \toprule
        \multirow{2}{3em}{\centering Vendor} & \multirow{2}{5em}{\centering Correctable Timing} & \multicolumn{5}{c}{Voltage}  \\
        \cmidrule(lr){3-7}
        & & 1.05 & 1.075 & 1.1 & 1.125 & 1.15  \\
        \midrule
        \multirow{3}{3em}{\centering A \\ \tiny 10 DIMMs \quad}
         & tRCD & - & - & 1/1 & - & - \\
         & tRP & - & - & - & - & - \\

        \cmidrule(lr){1-7}
        \multirow{3}{3em}{\centering B \\ \tiny 12 DIMMs \quad}
         & tRCD & 2/5 & 3/5 & 1/1 & 0 & 0 \\
         & tRP & 2/5 & 6/7 & 2/5 & 0/1 & - \\

        \cmidrule(lr){1-7}
        \multirow{3}{3em}{\centering C \\ \tiny 9 DIMMs \qquad}
         & tRCD & 0 & 0 & 0 & 3/4 & 3/3 \\
         & tRP & - & - & 0/1 & 0/5 & 0/5 \\
        \bottomrule
    \end{tabular}

  \caption{Performance results of memory non-intensive workloads with different
  \varr values.}
  \label{tab:non_mem_intensive_results}
\end{table}


==> sections/tables/motivation_freq_scaling.tex <==
\begin{table}[h]
%\reftiny
  \centering
    \setlength{\tabcolsep}{.35em}
    \begin{tabular}{ccccc}
        \toprule
        Workload & Speedup & Bandwidth & DRAM Energy & System Energy \\
        \midrule
        \emph{mcf} & \textbf{-19\%} & -20\% & -11\% & -2\% \\
        \emph{perl} & -2\% & -2\% & \textbf{-30\%} & -2\% \\
        \bottomrule
    \end{tabular}
  \caption{Workload behavior when the channel frequency reduces by half from
    1600 MT/s to 800 MT/s.}
  \label{tab:motivation}
\end{table}


==> sections/tables/mwork.tex <==
\definecolor{lightgray}{gray}{0.95}

\begin{table*}[h]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} &
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} &
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing}
\\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12}

 &
 & {\em \footnotesize (yy-ww)}
 & {\em \footnotesize Freq~(MT/s)}
 & {\em \footnotesize tRC (ns)}
 & {\em \footnotesize Size (GB)}
 & {\em \footnotesize Chips}
 & {\em \footnotesize Size (Gb)$^{\ddagger}$}
 & {\em \footnotesize Pins}
 & {\em \footnotesize Die Version$^{\S}$}
 & {\em \footnotesize tRP}
 & {\em \footnotesize tRCD} \\

\midrule

\cellcolor{white} & \module{A}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{A}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{A}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{A}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{A}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{A}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{A}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{A}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\multirow{-10}{5em}{\centering {\large\em A} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\

\cellcolor{white} & \module{A}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{A}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{A}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{A}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{A}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{A}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{A}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{A}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\multirow{-10}{5em}{\centering {\large\em A} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\

\cellcolor{white} & \module{A}{ 1}{} & 10-18 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 9.9  & 2.3	\\
\cellcolor{white} & \module{A}{ 2}{} & 10-20 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 23.4 & 440	\\
\cellcolor{white} & \module{A}{ 3}{} & 10-22 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 29   & 16.5	\\
\cellcolor{white} & \module{A}{ 4}{} & 10-23 & 1066 & 50.625 & 2 	& 8 & 2 & $\times$8  & $\mathcal{A}$ 	& 3.4  & 4.1	\\
\cellcolor{white} & \module{A}{ 5}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 11.2 \\
\cellcolor{white} & \module{A}{ 6}{} & 10-26 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.7  & 20.3 \\
\cellcolor{white} & \module{A}{ 7}{} & 10-43 & 1333 & 49.125 & 1 	& 8 & 1 & $\times$8  & $\mathcal{T}$ 	& 5837 & 764	\\
\cellcolor{white} & \module{A}{ 8}{} & 10-51 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 5.6  & 290  \\
\cellcolor{white} & \module{A}{ 9}{} & 11-12 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& --   & --   \\
\cellcolor{white} & \module{A}{10}{} & 11-19 & 1333 & 46.25  & 2 	& 8 & 2 & $\times$8  & $\mathcal{B}$ 	& 2.4  & 2.0  \\
\multirow{-10}{5em}{\centering {\large\em A} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{A}{30}{} & 13-11 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& 478  & 1590 \\

\bottomrule
\end{tabular}
%\input{tbl/module_legend}
%\caption{Sample Population of 30 DDR3 DIMMs from Vendor {\em A} (sorted by manufacturing date)}
%\label{tbl:vendor1}
\end{table*}

\ignore{
\definecolor{lightgray}{gray}{0.95}

\begin{table*}[t]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} &
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} &
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering \mycolorii{Vulnerability Ratio}$^{\star}$} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12}

 &
 & {\em \footnotesize (yy-ww)}
 & {\em \footnotesize Freq~(MT/s)}
 & {\em \footnotesize tRC (ns)}
 & {\em \footnotesize Size (GB)}
 & {\em \footnotesize Chips}
 & {\em \footnotesize Size (Gb)$^{\ddagger}$}
 & {\em \footnotesize Pins}
 & {\em \footnotesize Die Version$^{\S}$}
 & {\em \footnotesize tRP}
 & {\em \footnotesize tRCD} \\

\midrule

%% MICRON
\cellcolor{white} & \module{B}{ 1}{} & 10-09 & 1066 & 50.625 & 0.5& 4 & 1 & $\times$16 & $\mathcal{B}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 2}{} & 10-22 & 1066 & 50.625 & 0.5& 4 & 1 & $\times$16 & $\mathcal{B}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 3}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 4}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 5}{} & 10-23 & 1066 & 50.625 & 1  & 8 & 1 & $\times$8  & $\mathcal{F}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 6}{} & 11-26 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & --   & --   \\
\cellcolor{white} & \module{B}{ 7}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.1  & --   \\
\cellcolor{white} & \module{B}{ 8}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 479  & --   \\
\cellcolor{white} & \module{B}{ 9}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 1.9  & --   \\
\cellcolor{white} & \module{B}{10}{} & 11-35 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 4.3  & --   \\
\cellcolor{white} & \module{B}{11}{} & 12-02 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 161  & --   \\
\cellcolor{white} & \module{B}{12}{} & 12-02 & 1066 & 49.125 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 2.3  & --   \\
\cellcolor{white} & \module{B}{13}{} & 12-29 & 1600 & 50.625 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 16.0 & --   \\
\cellcolor{white} & \module{B}{14}{} & 12-29 & 1600 & 50.625 & 1  & 4 & 2 & $\times$16 & $\mathcal{D}$ & 8.6  & --   \\
\cellcolor{white} & \module{B}{15}{} & 12-26 & 1600 & 49.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{M}$ & --   & --   \\
\cellcolor{white} & \module{B}{16}{} & 12-26 & 1600 & 49.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{M}$ & --   & --   \\
\cellcolor{white} & \module{B}{17}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{18}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{19}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{20}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{21}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 4.3  & 11.4 \\
\cellcolor{white} & \module{B}{22}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 472  & --   \\
\cellcolor{white} & \module{B}{23}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 279  & --   \\
\cellcolor{white} & \module{B}{24}{} & 12-41 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 3276 & --   \\
\cellcolor{white} & \module{B}{25}{} & 13-02 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & --            & --   & --   \\
\cellcolor{white} & \module{B}{26}{} & 13-02 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & --            & --   & --   \\
\cellcolor{white} & \module{B}{27}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\cellcolor{white} & \module{B}{28}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 78.3 & 8.2  \\
\cellcolor{white} & \module{B}{29}{} & 13-33 & 1600 & 48.125 & 2  & 8 & 2 & $\times$8  & $\mathcal{K}$ & 23.4 & 5.8  \\
\multirow{-32}{5em}{\centering {\large\em B} \\ {\tiny \quad \\} \centering Total of \\ \centering 30 DIMMs}
\cellcolor{white} & \module{B}{30}{} & 14-09 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{K}$ & --   & --   \\
\bottomrule
\end{tabular}

\input{tbl/module_legend}

\caption{Sample Population of 30 DDR3 DIMMs from Vendor {\em B} (sorted by manufacturing date)}
\label{tbl:vendor2}
\end{table*}


\newpage

\definecolor{lightgray}{gray}{0.95}

\begin{table*}[t]

\setlength{\tabcolsep}{3pt}
\centering
\footnotesize

\begin{tabular}{cccccccccccc}

\toprule

\multirow{2}{*}[-2pt]{\em \footnotesize \centering Vendor} &
\multirow{2}{*}[-2pt]{\em \footnotesize \centering Module} &
                     {\em \footnotesize \centering Date$^{\ast}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Timing$^{\dagger}$} &
\multicolumn{2}{c}{\em \footnotesize \centering Organization} &
\multicolumn{3}{c}{\em \footnotesize \centering Chip} &
\multicolumn{2}{c}{\em \footnotesize \centering \mycolor{Vulnerability Ratio}$^{\star}$} \\

\cmidrule(lr){3-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12}

 &
 & {\em \footnotesize (yy-ww)}
 & {\em \footnotesize Freq~(MT/s)}
 & {\em \footnotesize tRC (ns)}
 & {\em \footnotesize Size (GB)}
 & {\em \footnotesize Chips}
 & {\em \footnotesize Size (Gb)$^{\ddagger}$}
 & {\em \footnotesize Pins}
 & {\em \footnotesize Die Version$^{\S}$}
 & {\em \footnotesize tRP}
 & {\em \footnotesize tRCD} \\

\midrule


%% SAMSUNG
\cellcolor{white} & \module{C}{ 1}{} & 08-49 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{D}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 2}{} & 09-49 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{E}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 3}{} & 10-19 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 4}{} & 11-16 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 5}{} & 11-19 & 1066 & 50.625 & 1 	& 8 & 1 & $\times$8  & $\mathcal{F}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 6}{} & 11-25 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{ 7}{} & 11-37 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 2.6  \\
\cellcolor{white} & \module{C}{ 8}{} & 11-46 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 32.9 \\
\cellcolor{white} & \module{C}{ 9}{} & 11-46 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 42.3 \\
\cellcolor{white} & \module{C}{10}{} & 11-49 & 1333 & 49.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{C}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{11}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 104  \\
\cellcolor{white} & \module{C}{12}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 117  \\
\cellcolor{white} & \module{C}{13}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 291  \\
\cellcolor{white} & \module{C}{14}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & --   \\
\cellcolor{white} & \module{C}{15}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 97.0 \\
\cellcolor{white} & \module{C}{16}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 493  \\
\cellcolor{white} & \module{C}{17}{} & 12-10 & 1866 & 47.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{D}$ 	& --   & 61.8 \\
\cellcolor{white} & \module{C}{18}{} & 12-25 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 2.2  & 3.3  \\
\cellcolor{white} & \module{C}{19}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 473  & 3.1  \\
\cellcolor{white} & \module{C}{20}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 5.4  & 2.7  \\
\cellcolor{white} & \module{C}{21}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 3.5  & 3.0  \\
\cellcolor{white} & \module{C}{22}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 545  & 3.0  \\
\cellcolor{white} & \module{C}{23}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 2.7  & 3.0  \\
\cellcolor{white} & \module{C}{24}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 27.2 & 2.9  \\
\cellcolor{white} & \module{C}{25}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 3.3  \\
\cellcolor{white} & \module{C}{26}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 54.2 & 19.1 \\
\cellcolor{white} & \module{C}{27}{} & 12-28 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 3.1  \\
\cellcolor{white} & \module{C}{28}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 29.0 & 5.4  \\
\cellcolor{white} & \module{C}{29}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 120  & 6.7  \\
\cellcolor{white} & \module{C}{30}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 196  & 3.2  \\
\cellcolor{white} & \module{C}{31}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 599  & 8.5  \\
\cellcolor{white} & \module{C}{32}{} & 12-31 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& 51.6 & --   \\
\cellcolor{white} & \module{C}{33}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 2.5  \\
\cellcolor{white} & \module{C}{34}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 1.6  \\
\cellcolor{white} & \module{C}{35}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 2.6  \\
\multirow{-38}{5em}{\centering {\large\em C} \\ {\tiny \quad \\} \centering Total of \\ \centering 36 DIMMs}
\cellcolor{white} & \module{C}{36}{} & 13-19 & 1600 & 48.125 & 2 	& 8 & 2 & $\times$8  & $\mathcal{E}$ 	& --   & 1.9  \\
\bottomrule
\end{tabular}

\input{tbl/module_legend}

\caption{Sample Population of 36 DDR3 DIMMs from Vendor {\em C} (sorted by manufacturing date)}
\label{tbl:vendor3}

\end{table*}
}


==> sections/tables/test.tex <==
%\reftiny

